Guaranteed Safe Reachability-based Trajectory Design for a High-Fidelity Model of an Autonomous Passenger Vehicle

Trajectory planning is challenging for autonomous cars since they operate in unpredictable environments with limited sensor horizons. To incorporate new information as it is sensed, planning is done in a loop, with the next plan being computed as the previous plan is executed. The recent Reachability-based Trajectory Design (RTD) is a provably safe, real-time algorithm for trajectory planning. RTD consists of an offline component, where a Forward Reachable Set (FRS) is computed for the vehicle tracking parameterized trajectories; and an online part, where the FRS is used to map obstacles to constraints for trajectory optimization in a provably-safe way. In the literature, RTD has only been applied to small mobile robots. The contribution of this work is applying RTD to a passenger vehicle in CarSim, with a full powertrain model, chassis and tire dynamics. RTD produces safe trajectory plans with the vehicle traveling up to 15 m/s on a two-lane road, with randomly-placed obstacles only known to the vehicle when detected within its sensor horizon. RTD is compared with a Nonlinear Model-Predictive Control (NMPC) and a Rapidly-exploring Random Tree (RRT) approach. The experiment demonstrates RTD's ability to plan safe trajectories in real time, in contrast to the existing state-of-the-art approaches.

==> sections/05_vehicle_RTD_implementation.tex <==
\section{Vehicle RTD Implementation}\label{sec:vehicle_rtd_implementation}

The main contribution of this paper is implementing RTD on a realistic passenger vehicle model in CarSim \cite{carsim}.
The Carsim model has 3 inputs: throttle position, brake pressure, and steering wheel angle.
This section has four parts.
First, we approximate the high-fidelity model via system identification, then use this approximate model to control the vehicle with linear MPC.
Second, we present the trajectory producing model.
Third, we find the error function $g$ as in Assumption \ref{ass:error_fn} using \eqref{prog:SOS_compute_g} to create the trajectory-tracking model and compute the FRS.
Fourth, we use the FRS for online planning.

\subsection{System Identification}\label{subsec:sys_ID}
We first approximate the high-fidelity model with an \emph{approximate model}, which occupies a state space $Z_\regtext{approx} \subset Z\hi$ such that $X \subset Z_\regtext{approx}$.
For this vehicle we use a bicycle model, similar to \cite[(1)]{liniger2017real}.
The approximate model consists of a simplified Pajecka model for the lateral tire forces, and polynomial functions relating the throttle and braking inputs to driving force.
To identify the model parameters, the CarSim model is run through a series of open-loop acceleration, and deceleration inputs to fit polynomial functions relating the throttle and brake inputs to the driving force, $F_x$.
This is used to identify a linear relationship between wheel angle, $\delta$, and steering wheel angle.
Cornering maneuvers produce data to fit a simplified Pajecka tire model to the lateral tire forces, $F_{f,y}$ and $F_{r,y}$.

The parameters for this model were fit by having the vehicle perform a variety of cornering, accelerating, and deceleration maneuvers.
This high-fidelity model is used: as the dynamic model in the trajectory tracking controller; to  predict the future state of the vehicle, during Algorithm X; and to aid in fitting the error function, $g$.

\subsection{Trajectory-Producing Model}\label{subsec:traj-prod_model_implem}
The reference trajectories passed to MPC are produced by the following trajectory-producing model (as in \eqref{eq:traj-producing_model}):


\subsection{Trajectory-Tracking Model and FRS Computation}\label{subsec:traj-track_and_FRS_implem}
